Visual Riddles: a Commonsense and World Knowledge Challenge for Large Vision and Language Models

Imagine observing someone scratching their arm; to understand why, additional context would be necessary. However, spotting a mosquito nearby would immediately offer a likely explanation for the person's discomfort, thereby alleviating the need for further information. This example illustrates how subtle visual cues can challenge our cognitive skills and demonstrates the complexity of interpreting visual scenarios. To study these skills, we present Visual Riddles, a benchmark aimed to test vision and language models on visual riddles requiring commonsense and world knowledge. The benchmark comprises 400 visual riddles, each featuring a unique image created by a variety of text-to-image models, question, ground-truth answer, textual hint, and attribution. Human evaluation reveals that existing models lag significantly behind human performance, which is at 82% accuracy, with Gemini-Pro-1.5 leading with 40% accuracy. Our benchmark comes with automatic evaluation tasks to make assessment scalable. These findings underscore the potential of Visual Riddles as a valuable resource for enhancing vision and language models' capabilities in interpreting complex visual scenarios.

==> figs_and_tables/fig_commonsense_categories.tex <==
\begin{figure}[!tb]
    \centering
    \includegraphics[width=\columnwidth]{images/category_model_performance.pdf}\\
\caption{\yb{The text is too small. Remove "Category Names" at the buttom}A histogram detailing the variety of commonsense knowledge required to solve the riddles in \datasetname{}. This knowledge spans a broad array of deviations from typical social norms and general knowledge. Additionally, the figure includes a comparative analysis of the explanation generation performance of the top two models from our experiments, as discussed in Section~\ref{section:Automatic_Evaluation_Experiments}. The left axis of the histogram indicates the frequency of each commonsense category, while the right axis shows the performance of both models.}
    \label{fig:fig_commonsense_categories}
\end{figure}

==> figs_and_tables/fig_question_creation.tex <==
\begin{figure}[!tb]
    \centering
    \includegraphics[width=\columnwidth]{images/Question Creation - Challenge Through Indirect Connection.pdf}\\
\caption{
Creating challenging question using indirect connection. First, challenge find the relevant clue that the question referring to in the image. Then, use world knowledge and commonsense regarding this clue in order to solve the question.}
    \label{fig:fig_qustion_creation}
\end{figure}

==> figs_and_tables/table_cannot_determine.tex <==
% \begin{table}[h]
% \caption{Excluding ``Cannot Determine'' Answer}
% \centering
% \setlength{\tabcolsep}{3pt}
% \begin{tabular}{lccccc}
% \hline
%  & \textbf{\% Accuracy $\uparrow$} & \textbf{ \% Cannot} & \textbf{\% Accuracy w/o} & \textbf{+ Hint $\uparrow$} & \textbf{+ Attribution $\uparrow$} \\
% & \textbf{} & \textbf{Determine} & \textbf{Cannot Determine} & & \\

% % \textbf{} & \textbf{Rating} & \textbf{\% Best Auto-Eval Model Rating} & \textbf{\% Best Auto-Eval Model Rating} & \textbf{\% Best Auto-Eval Model Rating} \\
% \hline 
% Gemini Pro 1.5    & 34 & 17 & 41 & 57 & 66 \\
% Gemini-Pro-Vision & 35 & 2 & 36 & 53 & - \\
% GPT4              & \textbf{39} & 12 & 44 & \textbf{59} & \textbf{75} \\
% LLaVA-1.5-7B      & 20 & 0 & 20 & 29 & - \\

% \hline
% \end{tabular}
% \label{table:cannot_determine_results}
% \end{table}



% \begin{table}[h]
% \caption{Accuracies Excluding ``Cannot Determine'' Answer}
% \centering
% \setlength{\tabcolsep}{3pt}
% \begin{tabular}{lcccccc}
% \hline
%  & \textbf{ \% Cannot} & \textbf{ \% Cannot Determine} & \textbf{ \% Cannot Determine} & \textbf{\% Accuracy w/o}  & \textbf{\% Accuracy + Hint } & \textbf{\% Accuracy + Attribution }\\
%  & \textbf{Determine}  & \textbf{ + Hint }             & \textbf{ + Attribution }      & \textbf{Cannot Determine} & \textbf{w/o Cannot Determine}& \textbf{w/o Cannot Determine} \\

% % \textbf{} & \textbf{Rating} & \textbf{\% Best Auto-Eval Model Rating} & \textbf{\% Best Auto-Eval Model Rating} & \textbf{\% Best Auto-Eval Model Rating} \\
% \hline 
% Gemini Pro 1.5    & 17 & 11 & 8 & 41 & 64 & 72\\
% Gemini-Pro-Vision & 2  & 1  &   & 36 & 54 & \\
% GPT4              & 1  & 0  & 2 & 20 & 29 & \textbf{76} \\
% LLaVA-1.5-7B      & 12 & 3  &   & 44 & 60 &\\

% \hline
% \end{tabular}
% \label{table:cannot_determine_results}
% \end{table}

==> figs_and_tables/table_evaluation_prompts.tex <==
% \begin{table}[h]
% \caption{Prompts for different models for Open-ended VQA Automatic Evaluation}
% \centering
% \begin{tabular}{l|p{10cm}}
% \hline

% \textbf{Task} & \textbf{Prompt}\\
% \hline
% Best Judge reference-free  & ``Answer with only Yes OR No. Given the image and the question, is the candidate answer correct?\nQuestion: $<question>$\nCandidate Answer: $<candidate\_answer>$\n''\\
% \hline
% Best Judge reference-based & ``Answer with only Yes OR No. Given the image, the question and the ground-truth answer, is the candidate answer correct?\nQuestion: $<question>$\nGround-Truth Answer:$<ground\_truth\_answer>$\nCandidate Answer: $<candidate\_answer>$\n'' \\ 
% \hline

% \hline
% \end{tabular}
% \label{table:EvaluationpromptExample}
% \end{table}

==> figs_and_tables/table_multiple_choice_prompts.tex <==
\begin{table}[h]
\caption{Prompts for different models for Multiple choice VQA task}
\centering
\begin{tabular}{l|p{10cm}}
\hline

\textbf{Task} & \textbf{Prompt}\\
\hline 
creating distractor & ``Here is a question regarding the image, and a ground-truth answer.\nQuestion:$<question>$\nGround-Truth Answer $<ground\_truth\_answer>$\n\nPlease generate $<num\_of\_incorrect\_distractors>$ wrong answers (that are kind-of similar to the ground-truth answer, and in a similar length) to the question based on the image, in the format of:\n\nYOUR FIRST ANSWER@@@YOUR SECOND ANSWER@@@...'' \\

\hline
Clean              & ``This is a multiple-choice question concerning the image. Out of the options labeled (1)-(5), only one is correct. Please provide your answer as a single digit that corresponds to the correct option. For instance, if the correct answer is (3), you should respond with 3.\n\nQuestion: $<question>$\n\nCandidate answers:\n(1)$<candidate1>$\n(2)$<candidate2>$ ...''\\

\hline
+ Hint             & ``This is a multiple-choice question concerning the image. Out of the options labeled (1)-(5), only one is correct. Please provide your answer as a single digit that corresponds to the correct option. For instance, if the correct answer is (3), you should respond with 3.\n\nQuestion: $<question>$\n\nHint: $<Hint>$\n\nCandidate answers:\n(1)$<candidate1>$\n(2)$<candidate2>$ ...''\\

\hline
+ Attribution      & ``This is a multiple-choice question concerning the image. Out of the options labeled (1)-(5), only one is correct. Please provide your answer as a single digit that corresponds to the correct option. For instance, if the correct answer is (3), you should respond with 3. Additionally, an attribution, which is a textual content from a webpage providing the basis for the correct answer, is also included below. Use this information to select the correct answer.\n\nQuestion: $<question>$\n\nAttribution:\n\verb|\|'\verb|\|'\verb|\|'\n$<attribution>$\n\verb|\|'\verb|\|'\verb|\|'\n\n\nCandidate answers:\n(1)$<candidate1>$\n(2)$<candidate2>$ ...''
\\
\hline

\hline
\end{tabular}
\label{table:MultiplePromptExample}
\end{table}

==> sections/6_related_work_backup.tex <==
\section{Related Work}
\label{sec:related_work}
% \yb{where is the related work? you can start adding the different links I sent you here}
% \yb{I was advised not to leave empty sections - consider adding something like This work is related to commonsense reasonning, factuality evaluation and attribution.. etc.}

Our research is closely linked to commonsense reasoning in multimodal models and the evaluation of factuality in both language-only and multimodal settings.

\paragraph{Commonsense reasoning in multimodal models.}
Recent progress in large multimodal models, including models like BLIP2 \cite{li2023blip}, Flamingo \cite{alayrac2022flamingo}, LLaVA \cite{liu2023llava}, GPT4 \cite{openai2024gpt4}, and Gemini-Pro \cite{team2023gemini}, have been pushing the boundaries of language-vision understanding.
 These developments have sparked interest in commonsense reasoning \cite{zellers2019recognition, vedantam2015learning}, leading to complex visual reasoning challenges within the vision-and-language domain.
These include specialized tests for understanding associations and analogies like WinoGAViL \cite{bitton2022winogavil} and VASR \cite{bitton2022vasr}, interpreting unusual images in WHOOPS! \cite{bitton2023breaking}, visual abductive reasoning tasks (e.g., Sherlock; \cite{hessel2022abduction}), multi-modal humor understanding tasks \cite{hessel2022androids}, and world-instructed image-editing tasks requiring commonsense reasoning (e.g., EditWorld;  \cite{yang2024editworld}).
Probably the closest benchmark to \datasetname{} is VisIT-Bench \cite{bitton2023visitbench}, where the authors took existing images and generated challenging questions about them. 
However, \datasetname{} distinguishes itself by allowing annotators more creative freedom to devise challenging scenarios and generate corresponding images and questions, rather than restricting them exclusively to what appears in the images.
This also ensures the images have not been previously seen during pretraining.

% \yb{Consider adding https://arxiv.org/pdf/2405.14785 as another example for a (very cool) work that uses generative images with commonsense relations. }

% \yb{It is good to add VisIT-Bench (You can remove the explicit mentions of WinoGAViL and VASR so it won't be obvious): https://visit-bench.github.io/, which has a similar concept, but with natural images. Then - my comment below will make more sense. In VisIT-Bench we started from existing images, and thought which challenging questions we can ask. The problem is that the existing image is limiting the thought - you cannot ask anything, just on what appears in the image. This could be a motivation for Visual Riddles} 

% \nitzan{+ the leaking problem of real images to training set of models}

% \datasetname{} sets itself apart by using synthetic images designed to depict specific scenarios with embedded visual clues to test models' ability to combine visual information with commonsense and world knowledge.

% \yb{Can highlight that we start with an idea in mind, and generate both an image and a challenging question to test it, rather than starting with existing image and ask questions about it.}



\paragraph{Factuality evaluation.}
There has been significant focus on evaluating factuality in language-only models, particularly in tasks where outputs are conditioned on grounding texts like summarization or machine translation. 
This area of research employs both reference-based metrics, such as Rouge \cite{lin2004rouge}, BLEU \cite{papineni2002bleu}, Bertscore \cite{zhang2019bertscore}, and COMET \cite{rei2020comet}, where generated text is compared to a reference, and reference-free metrics, such as SummaC \cite{laban2022summac}, Questeval \cite{scialom2021questeval}, $Q^2$ \cite{honovich-etal-2021-q2}, TRUE \cite{honovich2022true} and FiC \cite{slobodkin2024multi},  where the output is assessed against the input text(s).
Recently, there has been a similar move towards developing scalable and reliable metrics for factuality evaluation in vision-language tasks, including metrics like Clipscore \cite{hessel2021clipscore}, AVIBench \cite{zhang2024avibench}, and Tifa \cite{hu2023tifa}, and evaluation benchmarks such as MileBench \cite{song2024milebench}, SeeTRUE \cite{yarom2024you}, BLINK \cite{fu2024blink}, and Vibe-Eval \cite{padlewski2024vibe}. Our work introduces a complex factuality challenge requiring extensive world knowledge and substantial commonsense reasoning, demanding both information retrieval and critical analysis capabilities. Meanwhile, the Encyclopedic VQA \cite{mensink2023encyclopedic}, which also provides Wikipedia snippets for attribution, focuses primarily on world knowledge. In contrast, our dataset, \datasetname{}, adds layers of complexity by testing sensitivity to visual cues as well as commonsense reasoning, presenting a more demanding challenge.


% \yb{Will be good to mention what we are doing in this work -- we aim to ask questions that also posses a factuality challenge, where a solver (human or model) may be required to retrieve / find relevant information online, combining a reasoning challenge with a visual challenge.}

% \yb{Please also add Encyclopedic VQA: https://arxiv.org/abs/2306.09224. This is another motivator -- this paper did the factuality/attribution thing, but as the dataset is generated with retrieval methods (e.g., Wikipedia pages), there is only the retrieval / factuality challenge, and there is not a challenge in the visual clue -- finding a needle in a haystack that will allow to step towards solving the example}



% The field of commonsense reasoning has seen a surge of interest recently, spurring the development of numerous tasks across natural language processing (NLP) \cite{saha2021explagraphs, zellers2018swag, zellers2019hellaswag, sap2019atomic, bisk2020piqa, forbes2019neural} and computer vision \cite{vedantam2015learning, bitton2022vasr}. Within the vision-and-language domain, models are increasingly tasked with complex visual reasoning challenges. These tasks range from visual understanding, exemplified by VCR \cite{zellers2019recognition}, to more specialized tests of commonsense reasoning in scenarios requiring association and analogy, such as WinoGAViL \cite{bitton2022winogavil} and VASR \cite{bitton2022vasr}, or unique contexts like interpreting weird images \cite{bitton2023breaking} in WHOOPS!. Further, models are evaluated on their ability to conduct visual abductive reasoning (e.g., Sherlock; \cite{hessel2022abduction}) and to understand and explain multi-modal humor \cite{hessel2022androids}.
% Recent advancements in large language models, including BLIP2 \cite{li2023blip} and innovations in in-context and zero-shot learning approaches such as Flamingo \cite{alayrac2022flamingo} and MLLM \cite{https://doi.org/10.48550/arxiv.2302.14045}, are setting new standards for solving these intricate tasks. These developments underpin our work, which introduces a novel and challenging resource for evaluating AI models on visual riddles that require not only visual perception but deep commonsense and world-knowledge reasoning.

% \datasetname{} is distinct from prior work that focuses on reasoning with pre-existing images. Instead, it features synthetic images that depict specific scenarios with embedded visual clues designed to test AI models' ability to integrate commonsense, world-knowledge and visual information. By utilizing image generation models, we create unique and complex scenes that would otherwise be challenging to obtain, offering an opportunity to evaluate aspects of visual-reasoning, particularly in commonsense and world-knowledge applications.





% \begin{enumerate}
%     \item Multimodal Models for Image-Text Understanding
%     \item Commonsense reasoning - both generally in NLP and specifically in vision-language (including benchmarks and challenge sets).
%     \item attributed text generation.
%     \item evaluation of instruction-following and factuality (both only language and language-vision)
    
% \end{enumerate}








==> sections/deprecated_introduction.tex <==
% \yb{hi}, \nitzan{hi}, \aviv{hi}, \eliya{hi}, \aviya{hi}, \royi{hi}, \amir{hi}, \idan{hi}

Upon observing a visual scene, humans effortlessly interpret complex elements and incongruities through a lens of commonsense reasoning — a capacity that current vision and language models not always manage to perfectly replicate. Consider a seemingly ordinary scenario where a person scratches his arm; this action gains new significance when contextualized with a mosquito visible on the nearby nightstand. \aviv{combined with the abstract, the mosquito example feels repetitive - maybe omit it from the abstract?} While such nuances are readily deciphered by humans, machines can find it challenging to connect these visual clues to broader world knowledge and commonsense, that derived from
cultural aspects, life-experiences and even physical or social knowledge~\cite{sap2019socialiqa,zellers2019recognition,hessel2022androids,talmor2022commonsenseqa}.

\yb{Missing information. Please add another paragraph here that explains (1) why it is important to understand and make progress on this task (search for our previous works in Winogavil and WHOOPS!); (2) List previous works, including BLINK, and some new ones, but mention that their limitation is on natural images and find a way to say that the question comes after the image is created; (3) Motivate our novelty: we wanted to first come with idea in mind, and then create an image that challenges this concept in an isolated and concise way}

In this work, we introduce \datasetname{}, a dataset comprising \datasetinstancesnumber{} visual riddles, each consisting of a synthetic image, a question, and an answer designed to challenge AI models beyond traditional recognition tasks. These visual riddles require models to not only identify visual clues but also to understand their relevance to the presented question and formulate answers that draw on commonsense and world knowledge.
To create \datasetname{}, we collaborated with designers who utilized advanced text-to-image models like Midjourney, Ideogram, Canva, \dalle{} \cite{ramesh2021zero}, and Stable-Diffusion \cite{rombach2022high}. These tools generate images that embed crucial visual clues necessary for solving the riddles, an approach essential for depicting scenarios that are difficult to capture through conventional image collection methods. The designers crafted challenges that integrate both visual and commonsense clues to test the models' interpretive abilities comprehensively.
Additionally, to make our challenge set more comprehensive and to enable the creation of easier tasks, designers included supplementary data such as hints, which direct attention to visual clues in the image, and attributions, which are web sources confirming the validity of the answers. Figure~\ref{fig:fig1} illustrates two examples. The first riddle shows a man scratching his arm due to a mosquito bite, where the presence of the mosquito is the key clue, highlighting the need for strategic visual clues. The second riddle features a person eating soup, where recognizing the person is in Japan is just the first step; web searches are needed to learn that eating soup directly from the bowl is polite in Japan.


% Figure~\ref{fig:fig1} that present the riddle from our challenge set that presenting a man scratching his arm due to a mosquito bite. The key to solving this riddle—the presence of the mosquito—highlights the necessity of placing visual clues strategically within the image to guide the model towards the correct solution. Sometimes, identifying the visual clue alone is insufficient to solve the riddle. For instance, in the second example in Figure~\ref{fig:fig1}, recognizing that the person is in Japan is only the first step. To fully answer the riddle, one must also use web searches to learn about local dining etiquette, specifically how it is polite to eat soup in Japan.\yb{the last part of the examples are good, you can just write them more concisely (we can address it later)}


Next, we pose three visual commonsense reasoning tasks
over the \datasetname{} riddles: (1) open-ended,
where models need to solve a visual riddle consists of an image and a question in three settings - without using additional data, using hints, and using attribution; (2) multiple-choice, where models need to select the correct answer for the riddle out of 5 possible answers. The main purpose of this task is to enable fully automatic evaluation using a simple accuracy metric; (3) automatic-evaluation, where models need to evaluate if an answer for a riddle is correct in two setting - reference-free, without additional information and reference-based - with the ground-truth answer as a reference. The main objective of this task is to identify the best auto-rater for evaluating the performances of models on open-ended visual riddles (Figure~\ref{fig:fig_tasks}). Our evaluation of these tasks aimed at assessing different facets of the models' reasoning capabilities.

Experimental results from the Visual Riddles challenge illustrate a substantial performance disparity between humans and state-of-the-art vision and language models like LLaVA, Gemini-Pro-Vision, Gemini-Pro-1.5, InstructBlip, and GPT-4. Humans successfully solved 83\% of the visual riddles, while Gemini-Pro-1.5 achieved 42\% and GPT-4 only 32\%. In multiple-choice selections, models performed better than in the open-ended tasks, with GPT-4 leading at 55\%, followed by Gemini-Pro-1.5 at 47\%, and all other models below 44\%. To facilitate fully automated evaluations, we conducted experiments on these models in both reference-free and reference-based settings, comparing their performance with human ratings. In the reference-based scenario, Gemini-Pro-1.5 achieved 85\% alignment with human ratings, making it suitable as an auto-rater. Using this auto-rater, further experimentation demonstrated that although models show marginally better performance when provided with hints and attributions, significant challenges remain. For instance, GPT-4's accuracy rose to 62\% with attributions and 55\% with hints. 


Additionally, our analysis shows that models do not recognize enough visual clues to determine if a candidate answer is correct. Our evaluation of text-to-image models reveals that only X\% of generated images accurately conveyed the expected commonsense idea, underscoring the dataset's challenge and the need for strategic visual clues. Furthermore, the necessity of a manual process to create the \datasetname{} images is evident, as only 15\% of images generated with the same prompts were equivalent and suitable replacements for the original images in the visual riddles.


Overall, the findings suggest that the \datasetname{} poses a formidable challenge even to state-of-the-art vision-and-language models. These results underscore the critical need for ongoing advancements in commonsense reasoning and the integration of world knowledge to enhance the models' capabilities in tackling complex visual riddles; Data, code
and leaderboard are available at \url{https://visual-riddles.github.io/}.


\begin{figure}[!tb]
    \centering
    \includegraphics[width=\columnwidth]{images/Tasks2.pdf}\\
\caption{
Overview of tasks in the \datasetname{} benchmark. (1) Primary Task: Solving visual riddles composed of images and open-ended questions. (2) Utilizing Hints: Solving visual riddles with textual aids to identify key visual clues. (3) Employing Attributions: Using web-sourced attributions to provide necessary commonsense knowledge for riddle resolution. (4) Multiple Choice: Choosing the correct answer from five options to test discernment and accuracy. (5) Automatic Evaluation: Conducting evaluations in two scenarios—Reference-Free, to determine the correctness of a candidate answer based solely on the visual riddle, and Reference-Based, to assess alignment with the ground truth.
}
    \label{fig:fig_tasks}
\end{figure}
